Fearless Stochasticity in Expectation Propagation

Expectation propagation (EP) is a family of algorithms for performing approximate inference in probabilistic models. The updates of EP involve the evaluation of moments -- expectations of certain functions -- which can be estimated from Monte Carlo (MC) samples. However, the updates are not robust to MC noise when performed naively, and various prior works have attempted to address this issue in different ways. In this work, we provide a novel perspective on the moment-matching updates of EP; namely, that they perform natural-gradient-based optimisation of a variational objective. We use this insight to motivate two new EP variants, with updates that are particularly well-suited to MC estimation. They remain stable and are most sample-efficient when estimated with just a single sample. These new variants combine the benefits of their predecessors and address key weaknesses. In particular, they are easier to tune, offer an improved speed-accuracy trade-off, and do not rely on the use of debiasing estimators. We demonstrate their efficacy on a variety of probabilistic inference tasks.

==> relatedwork.tex <==
\section{Related Work}
\label{sec:relatedwork}

% In this setting, EP can be viewed as a divide-and-conquer style method, with one large inference problem being separated into several smaller MCMC tasks. These tasks interact through the site parameters, which convey information about the global density, and are then used to focus local sampling efforts on the regions of high global density. This approach which, has potential for significant computational savings over conventional MCMC methods (see Appendix \ref{app:epbenefits}), was used by \citet{xu2014sms} in a method called \textit{sampling via moment sharing} (SMS), and later by \citet{vehtari2020} in the context of hierarchical models. However, several challenges remain.



% \begin{enumerate}
%     \item SMS
%     \item SNEP
%     \item EP as a way of life
%     \item Consensus MCMC
%     \item Embarassingly parallel MCMC
%     \item Weierstrass sampler
% \end{enumerate}
